MitoWorld: A Stochastic World Model of the Single-Cell Cycle under Genetic Perturbation

A cell observed after a gene knockdown has an uncertain future, both in how its appearance will evolve and when it will divide. Existing approaches predict endpoints or population-level changes without jointly modeling individual trajectories and division timing. In this work, we present MitoWorld, a stochastic world model that generates these future appearances as continuous evolution in a Gaussian reference latent, terminated by a division hazard and converted into images by a conditional diffusion renderer. The ordinary transition provably preserves its Gaussian reference, tying its noise to its dynamics; paired observations identify its discrete transition where stationary marginals cannot. The hazard turns division timing into a survival likelihood that can be tested against real cycle lengths. On 325 held-out MitoCheck tracks spanning 17 knockdowns and a control, MitoWorld lowers FID by 34.6\% and the video metric JEDi by 45.6\% relative to the strongest baselines. Its latent-space prediction intervals achieve near-nominal 90\% coverage, are 35\% narrower than those of a model with freely fitted noise. The hazard also yields cell-cycle length distributions with KS distance close to the model-based finite-sample reference. Testable single-cell stochastic dynamics thus offer a generative tool for time-lapse perturbation screens.

==> figure/main/04_02_per_cell_prediction/fig3_snapshots_a.tex <==
% Six selected snapshots per row. Ages/source continuity are specified in caption/provenance.
\begin{tikzpicture}[x=1cm,y=1cm,font=\small,
  methodlabel/.style={anchor=east,inner sep=0pt,font=\fontsize{15}{18}\selectfont}]
  \path[use as bounding box] (0,-10.18) rectangle (17.8,1.40);
  \node[anchor=west,inner sep=0pt] at (3,0)
    {\includegraphics[width=14.8cm]{figure/main/04_02_per_cell_prediction/rollout_selected_20261103/real.png}};
  \node[anchor=west,inner sep=0pt] at (3,-2.67)
    {\includegraphics[width=14.8cm]{figure/main/04_02_per_cell_prediction/rollout_selected_20261103/impa.png}};
  \node[anchor=west,inner sep=0pt] at (3,-5.34)
    {\includegraphics[width=14.8cm]{figure/main/04_02_per_cell_prediction/rollout_selected_20261103/hi.png}};
  \node[anchor=west,inner sep=0pt] at (3,-8.01)
    {\includegraphics[width=14.8cm]{figure/main/04_02_per_cell_prediction/rollout_selected_20261103/mitoworld.png}};
  \foreach \row/\label in {0/Observed,1/IMPA,2/HI,3/MitoWorld} {
    \ifnum\row=3
      \node[methodlabel,text=black,font=\fontsize{15}{18}\selectfont\bfseries] at (2.85,{-2.67*\row}) {\label};
    \else
      \node[methodlabel,text=black] at (2.85,{-2.67*\row}) {\label};
    \fi
  }
  \shade[left color=black!12,right color=black!82]
    (3,-9.88) -- (15.65,-9.88) -- (15.65,-10.05) -- (16.10,-9.75)
    -- (15.65,-9.45) -- (15.65,-9.62) -- (3,-9.62) -- cycle;
  \node[anchor=west,inner sep=0pt,font=\fontsize{15}{18}\selectfont]
    at (16.35,-9.75) {Time};
\end{tikzpicture}

